Zoology: Measuring and Improving Recall in Efficient Language Models

Attention-free language models that combine gating and convolutions are growing in popularity due to their efficiency and increasingly competitive performance. To better understand these architectures, we pretrain a suite of 17 attention and "gated-convolution" language models, finding that SoTA gated-convolution architectures still underperform attention by up to 2.1 perplexity points on the Pile. In fine-grained analysis, we find 82% of the gap is explained by each model's ability to recall information that is previously mentioned in-context, e.g. "Hakuna Matata means no worries Hakuna Matata it means no" $\rightarrow$ "??". On this task, termed "associative recall", we find that attention outperforms gated-convolutions by a large margin: a 70M parameter attention model outperforms a 1.4 billion parameter gated-convolution model on associative recall. This is surprising because prior work shows gated convolutions can perfectly solve synthetic tests for AR capability. To close the gap between synthetics and real language, we develop a new formalization of the task called multi-query associative recall (MQAR) that better reflects actual language. We perform an empirical and theoretical study of MQAR that elucidates differences in the parameter-efficiency of attention and gated-convolution recall. Informed by our analysis, we evaluate simple convolution-attention hybrids and show that hybrids with input-dependent sparse attention patterns can close 97.4% of the gap to attention, while maintaining sub-quadratic scaling. Our code is accessible at: https://github.com/HazyResearch/zoology.

==> Figures/Main/Figure3/figure.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{Figures/Main/Figure3/data_dependent.png}
    \caption{\textbf{Data dependent convolutions and accuracy on associative recall.} The x-axis is the model dimension and the y-axis is accuracy. There are many methods to introduce data-dependent shifts to an architecture. We observe any of our convolution-architectures with data-dependent shifts outperforms the gated convolutions with data-independent shifts across settings. (\yell{plot captured while some runs are in progress})}
    \label{fig:datadep}
    \vspace{-2mm}
\end{figure}


==> Tables/downstream_extended.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
 &  &  & \textbf{Overall} & \multicolumn{2}{c}{\textbf{Slices}} & \textbf{\% of gap due to} \\ 

Model (Window Size) & Param (M) & TFLOPs  & & AR Hits & Other Tokens & AR Hits\\
\midrule
Attention & 125 & 2.46 & \textbf{11.01} (2.40) & \textbf{2.16 (0.77)} & 12.45 (2.52) & ---  \\
\midrule
RetNet (128) & 152 & 2.60 & 11.15 (2.41) & 3.01 (1.10) & 12.45 (2.55) & 100\% \\
\midrule
Hyena     & 160 & 2.41 &   11.60 (2.45) & 5.00 (1.61) & 12.28 (2.51) & 100\% \\
 + Sliding Attn. (64) & 159 & 2.28 &  11.57 (2.45) &  5.23 (1.65) &  12.30 (2.51) & 100\% \\
 + Sliding Attn. (256) & 159 & 2.29 & \textbf{10.65} (2.37) &  3.42 (1.23) &  11.52 (2.45) & 100\% \\
\bottomrule
\end{tabular}
\caption{\textbf{Language modeling validation perplexity on the Pile.} After pretraining on 10B tokens of Pile data, we report log perplexity with negative log-likelihood in parentheses. We report overall scores, and for the AR vs. non-AR token slices defined in \Cref{sec:sec3-downstream}. FLOPs are computed for inputs of 2048 tokens based on the equations in Appendix \ref{app:expdetails}.
}
\label{table:extra-ppl-slices}
\end{table}



==> Tables/downstream_hyena.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
 &  &  & \textbf{Overall} & \multicolumn{2}{c}{\textbf{Slices}} & \textbf{\% of gap due to} \\ 

Model ($w$ Sine Freq.) & Param (M) & TFLOPs  & & AR Hits & Other Tokens & AR Hits\\
\midrule
Attention & 125 & 2.46 & \textbf{11.01} (2.40) & \textbf{2.16 (0.77)} & 12.45 (2.52) & ---  \\
Attention & 360 & 6.23 &  \textbf{9.44} (2.25) & \textbf{1.98 (0.69)} & 10.62 (2.36) &  ---  \\
\midrule
Hyena ($w=14$) & 158 & 2.41 &   11.60 (2.45) & 5.00 (1.61) & 12.28 (2.51) & 100\% \\
Hyena ($w=2$) & 158 & 2.41 & 11.47 (2.44) & 4.63 (1.53) & 12.30 (2.51) & 100\% \\
+ 4 Heads & 150 & 2.47 & 11.05 (2.40) & 3.47 (1.24) & 12.07 (2.49) &  100\% \\
\midrule
Hyena ($w=14$) & 358 & 5.03 & 10.07 (2.31) & 3.83 (1.34) & 10.75 (2.38) & 98.2\% \\
Hyena ($w=2$) & 358 & 5.03 & 9.86 (2.29) & 3.46 (1.24) & 10.69 (2.37) & 100\% \\
+ 4 Heads & 358 & 5.18 & 9.48 (2.25) & 2.78 (1.02) & 10.42 (2.34) & 100\% \\
\bottomrule
\end{tabular}
\caption{\textbf{Language modeling validation perplexity on the Pile.} After pretraining on 10B tokens of Pile data, we report log perplexity with negative log-likelihood in parentheses. We report overall scores, and for the AR vs. non-AR token slices defined in \Cref{sec:sec3-downstream}. FLOPs are computed for inputs of 2048 tokens based on the equations in Appendix \ref{app:expdetails}. Here we evaluate Hyena at two different hyperparameter settings and in the multi-head setting. 
}
\label{table:extra-hyena}
\end{table}


==> Tables/pile.tex <==
\begin{table}[t]
    \caption{Test perplexity on the PILE when trained for different amounts of tokens. }
    \label{tab:the_pile}
    \centering
    \begin{tabular}{rccccc} \toprule
    {Model} & 5B & 10B & 15B & Description\\ \midrule
    Transformer (125M) & & \yell{10.5} & & Llama MLP, Learned Embedding \\
    Llama Transformer (125M) & \yell{12.6} & 11.2 & & Llama MLP, Rotary Embedding  \\
    Hyena (155M) & \yell{13.5} & 12.0 &  & \\
    Ours - Dyadic & &  &  & \\
    Ours - Sparse Attn. (155M) & \textbf{\yell{12.3}} & \textbf{10.9} & & \\
    \midrule
    \bottomrule 
    \end{tabular}
\end{table}



==> macros.tex <==
\newcommand{\assume}[1]{#1}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}

%% OPERATORS:
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
\newcommand{\argmin}[2]{\textrm{argmin}_{#1}~#2}
\newcommand{\argmax}[2]{\textrm{argmax}_{#1}~#2}
% Inner product
\newcommand{\ip}[2]{\left\langle#1, #2\right\rangle}
% Trace
\newcommand{\tr}{\textrm{tr}}
% Expected value
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
% Sample mean
\newcommand{\Ehat}[1]{\hat{\mathbb{E}}\left[#1\right]}
% Variance
\newcommand{\Var}[2]{\textrm{Var}_{#1}\left[#2\right]}
% Covariance
\newcommand{\Cov}[2]{\textrm{\textbf{Cov}}_{#1}\left[#2\right]}
% Indicator
\newcommand{\ind}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\indpm}[1]{\mathbbm{1}^{\pm}\left\{#1\right\}}
% sech
\newcommand{\sech}[0]{\textrm{sech}}
% diag
\newcommand{\diagm}[1]{\textrm{diagm}\left(#1\right)}
% supp
\newcommand{\supp}{\text{supp}}
% independent
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\bp}{q}

%\newenvironment{bsmallmatrix}
%  {\left[\begin{smallmatrix}}
%  {\end{smallmatrix}\right]}
\usepackage[dvipsnames]{xcolor}
\usepackage{xargs}

% see line at top of main file to show/hide notes
\ifdefined\ShowNotes
  \newcommand{\colornote}[3]{{\color{#1}\bf{#2 #3}\normalfont}}
\else
  \newcommand{\colornote}[3]{}
\fi

\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{darkgreen}{rgb}{0.1,0.5,0.1}
\definecolor{cyan}{rgb}{0.7,0.0,0.7}
\definecolor{dblue}{rgb}{0.2,0.2,0.8}
\definecolor{maroon}{rgb}{0.76,.13,.28}
\definecolor{burntorange}{rgb}{0.81,.33,0}
\definecolor{royalpurple}{rgb}{0.47,.31,0.66}
\definecolor{greenn}{rgb}{0.1,0.5,0.3}
\definecolor{purplee}{rgb}{0.5,.31,0.8}

% \newcommand {\note}[1]{\colornote{maroon}{}{#1}}
\newcommand {\todo}[1]{\colornote{cyan}{TODO}{#1}}
\newcommand {\dan}[1]{\colornote{darkgreen}{DF:}{#1}}
\newcommand {\simran}[1]{\colornote{burntorange}{SA:}{#1}}
\newcommand {\sabri}[1]{\colornote{red}{SE:}{#1}}
\newcommand {\atri}[1]{\colornote{burntorange}{Atri:}{#1}}
\newcommand {\armin}[1]{\colornote{royalpurple}{Armin:}{#1}}
\newcommand {\isys}[1]{\colornote{greenn}{Isys:}{#1}}
\newcommand {\jess}[1]{\colornote{purplee}{Jess:}{#1}}
\newcommand {\tri}[1]{\colornote{blue}{TD:}{#1}}
% To hide comments:
%\newcommand {\tri}[1]{}

% not a colornote since we don't want these to ever be removed from the document
\ifdefined\ShowNotes
  \newcommand{\num}[1]{{\color{red}\bf{#1}\normalfont}}
\else
  \newcommand{\num}[1]{#1}
\fi

\newcommand{\sysname}{\textsc{Monarch Mixer}\xspace}
\newcommand{\sysabbrev}{\textsc{M2}\xspace}

% MP: dingbats
\usepackage{pifont}
\newcommand{\xmark}{\ding{55}}%
